Comparison of Macro- and Microscopic Solutions of the Riemann Problem II. Two-Phase Shock Tube

The Riemann problem is one of the basic building blocks for numerical methods in computational fluid mechanics. Nonetheless, there are still open questions and gaps in theory and modelling for situations with complex thermodynamic behavior. In this series, we compare numerical solutions of the macroscopic flow equations with molecular dynamics simulation data. To enable molecular dynamics for sufficiently large scales in time and space, we selected the truncated and shifted Lennard-Jones potential for which also highly accurate equations of state are available. A comparison of a two-phase Riemann problem is shown, which involves a liquid and a vapor phase, with an undergoing phase transition. The loss of hyperbolicity allows for the occurrence of anomalous wave structures. We successfully compare the molecular dynamics data with two macroscopic numerical solutions obtained by either assuming local phase equilibrium or by imposing a kinetic relation and allowing for metastable states.

==> packages.tex <==
\RequirePackage{etex}
\usepackage{etoolbox}  % insert new e-TEX commands (required for \AfterEndEnvironment)

%-------------------------------------------------------------------------------
% EQUATIONS
%-------------------------------------------------------------------------------
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amscd}
\usepackage{amsfonts}
\usepackage{breqn}
\usepackage{mathtools}
\usepackage{nicefrac}
\usepackage[llbracket,rrbracket]{stmaryrd}
\usepackage[normalem]{ulem}

%-------------------------------------------------------------------------------
% COLOURS
%-------------------------------------------------------------------------------
\usepackage{xcolor}

%\definecolor{myblue}{RGB}{68,119,170}
%\definecolor{mycyan}{RGB}{102,204,238}
%\definecolor{mygreen}{RGB}{34,136,51}
%\definecolor{myyellow}{RGB}{204,187,68}
%\definecolor{myred}{RGB}{238,102,119}
%\definecolor{mypurple}{RGB}{170,51,119}
%\definecolor{mygrey}{RGB}{187,187,187}

\definecolor{myblue}{RGB}{0,119,187}
\definecolor{mycyan}{RGB}{51,187,238}
\definecolor{mygreen}{RGB}{0,153,136}
\definecolor{myyellow}{RGB}{238,119,51} % this is acutally orange
\definecolor{myred}{RGB}{204,51,17}
\definecolor{mypurple}{RGB}{238,51,119} % this is acutally magenta
\definecolor{mygrey}{RGB}{187,187,187}

%-------------------------------------------------------------------------------
% TABULAR
%-------------------------------------------------------------------------------
%\usepackage{supertabular}
%\usepackage{array}
%\usepackage{longtable}
\usepackage{tabularx}
%\renewcommand{\arraystretch}{1.1}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs} % The package enhances the quality of tables

%-------------------------------------------------------------------------------
% CAPTIONS
%-------------------------------------------------------------------------------
\usepackage[format=hang,labelfont=bf]{caption}  % Tabellen/Figure Beschriftung 
\usepackage{subcaption}

% -------------------------------------------------------------------------------
% SI units
% -------------------------------------------------------------------------------
\usepackage{siunitx}
%\sisetup{inter-unit-product =$\cdot$}
\sisetup{exponent-product = \cdot, output-product = \cdot}
%\sisetup{detect-weight, detect-display-math}
%\sisetup{detect-inline-weight=math}
\sisetup{allow-number-unit-breaks}

% Angstrom symbol
\DeclareSIUnit{\angstrom}{\mbox{\normalfont\AA}}
\makeatletter
\DeclareRobustCommand{\AA}{%
  \leavevmode
  \vbox{\ialign{##\cr
    \hidewidth\char'27 \hidewidth\cr
    \noalign{\nointerlineskip\kern-1.4ex}
    A\cr
  }}%
}
\makeatother


%------------------------------------------------------------------------------
% References 
%------------------------------------------------------------------------------
\usepackage[capitalise]{cleveref}

%-------------------------------------------------------------------------------
% OTHER USEFUL PACKAGES
%-------------------------------------------------------------------------------
\usepackage{changebar}
\usepackage[mode=image]{standalone}
\usepackage{csquotes}  % Anfuehrungszeichen (wird von glossaries empfohlen)
\usepackage{xspace}    % Leerzeichen oder nicht nach Kommando einfuegen

\usepackage[all]{nowidow} % Witwen und Waisen (Hurenkinder, Schusterjungen) vermeiden

\frenchspacing % No big horizontal spaces between sentences


